BRI3L: A Brightness Illusion Image Dataset for Identification and Localization of Regions of Illusory Perception

Visual illusions play a significant role in understanding visual perception. Current methods in understanding and evaluating visual illusions are mostly deterministic filtering based approach and they evaluate on a handful of visual illusions, and the conclusions therefore, are not generic. To this end, we generate a large-scale dataset of 22,366 images (BRI3L: BRightness Illusion Image dataset for Identification and Localization of illusory perception) of the five types of brightness illusions and benchmark the dataset using data-driven neural network based approaches. The dataset contains label information - (1) whether a particular image is illusory/nonillusory, (2) the segmentation mask of the illusory region of the image. Hence, both the classification and segmentation task can be evaluated using this dataset. We follow the standard psychophysical experiments involving human subjects to validate the dataset. To the best of our knowledge, this is the first attempt to develop a dataset of visual illusions and benchmark using data-driven approach for illusion classification and localization. We consider five well-studied types of brightness illusions: 1) Hermann grid, 2) Simultaneous Brightness Contrast, 3) White illusion, 4) Grid illusion, and 5) Induced Grating illusion. Benchmarking on the dataset achieves 99.56% accuracy in illusion identification and 84.37% pixel accuracy in illusion localization. The application of deep learning model, it is shown, also generalizes over unseen brightness illusions like brightness assimilation to contrast transitions. We also test the ability of state-of-theart diffusion models to generate brightness illusions. We have provided all the code, dataset, instructions etc in the github repo: https://github.com/aniket004/BRI3L

==> supple.tex <==
\section{Supplementary Material}

In the supplementary material, we are providing the following details.
\begin{enumerate}
    \item Details of psychophysical experiments and results.
    \item Details of dataset generation.
    \item Networks details for illusion detection and localization.
    \item More qualitative experimental results.
    \item Generalization to unseen illusions.
    \item Illusion vs natural images.
    \item Test on illusions in natural images.
    \item Network analysis.
\end{enumerate}


\section{Psychophysical Experiment – Detail experimental setup, procedure and result.}


\subsection{Background}

Gustav Theodor Fechner~\cite{fechner18601966} was the pioneer to set  the principles and procedures of psychophysics. It is a sub-discipline  of psychology and deals with the relationship between physical stimuli and their subjective correlates or percepts.
In different intensity based visual illusions, the lightness of the test patch is modified which is termed as illusory effect. This illusory effect is subjective in nature. Performing comparison of the intensity of the test patch with a standard patch of known intensity, one can only guess whether the test patch is lighter or darker as compared with the standard. Psychophysical experiments are designed to measure the illusory effect quantitatively and can also judge the direction of the illusory effect.


A psychophysical experiment consists of a number of components like stimulus (comparator and standard), task, method, analysis and measure. Two types of procedures exist in psychophysical experiments. In the first type, the comparator is displayed on the computer screen and the observer has to adjust the contrast within a predefined limit to achieve the perceivable intensity as compared with the standard. For this type of procedure, the task and the method are collectively termed as `method of adjustment'.
Nowadays the preferred approach is to display the comparator and standard in a random fashion on a computer screen for a short duration of time. The observer has to decide the relative brightness of the comparator with respect to that of the standard and indicate his/her choice by pressing a key. This is known as 2 Alternate Forced Choice (2AFC) experiment~\cite{mitra2018adaptive}.


Four types of intensity based illusions namely, Simultaneous Brightness Contrast(SBC), White Illusion (WI), Gratings and Lower Grid illusions with variable parameters ( say length, width, intensity background etc.) are generated randomly and the darker patch is selected as the target patch or comparator.
The two alternate forced choice (2AFC) experimental setup has been adopted to quantify the illusory enhancement or reduction of the selected target patch. The psychometric curve is drawn in Fig. 4 (in the paper) and Fig.~\ref{fig:psychometric_curve_supp} for a specific illusion and the illusory effect of the test patch is quantified at the point of subjective equality (PSE).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[scale=0.3]{figures/exp_1.png}
%\vspace{-0.2cm}
\caption{Different types of SBC illusions selected as the comparator. The intensity level of the target is always 150. However the length and width of the target varies widely.}
%\vspace{-0.2cm}
\label{fig:exp_setup_supp}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
\centering
% \includegraphics[scale=0.38]{figures/ill_curve.png}
\includegraphics[scale=0.35]{figures/psycho_curve.png}
%\vspace{-0.5cm}
\caption{Psychometric curve for (a)Lower grid, (b) SBC, (c) White illusion, (d) Grating illusion taken from the generated dataset.
This indicates the probability that the perception agrees with the reality as a function of the real difference in luminance between the standard (S) and the comparator (C).
The illusory reduction for Grating, White illusion, SBC, Lower grid are 26.69, 49.22, 35.03 and 32.95 respectively. }
%\vspace{-0.2cm}
\label{fig:psychometric_curve_supp}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Materials and Methods}

The experimental arrangements are designed identical to that described in Mitra et al.~\cite{mitra2018adaptive} and Shi et al.~\cite{shi2013effect}. A chin rest is placed at a distance of d cm from a linearized video monitor (HP Compaq LE 2002X with resolution 1,024 X 1,024 pixels) and the subject’s head is stabilized on this chin rest. The value of d is chosen as 57 cm, because it may be shown from simple trigonometry that at such a distance an image of width (or length) of one cm. subtends a visual angle of approximately 1 degree. Subjects binocularly view the visual presentations, keeping their heads fixed on the chin rest.
In these experiments, the subjects visually compare the brightness or lightness of two targets, namely the standard and the comparator. We conduct a two-alternative forced-choice experiment for lightness discrimination between the comparator and the standard and measured the illusory enhancement or illusory reduction. The subjects are instructed to give his/her judgment by pressing the key marked ONE when the comparator appeared to be lighter than the standard, otherwise key marked as TWO was to be pressed.
The comparator is an intensity based illusion generated statistically and it is selected individually from four types of illusions namely Simultaneous Brightness Contrast (SBC), White Illusion (WI), Gratings and Lower Grid illusions. 
In one set of experiment, the same type of the illusion, say SBC illusion is selected as the comparator. One such set of SBC illusion is shown in Fig.~\ref{fig:exp_setup_supp}. The intensity level of the target remains always 150, however it appears either lighter or, darker depending on the background intensity. In all the trials, the darker target is selected as the comparator, whose intensity is compared with the standard.


In our experiments, the standard is a target, containing a number of segments. Each segment could be distinguished from the other by its intensity of gray value. For example, our striped standard was divided into 11  segments of varying intensity values values 13, 36, 59, 82, 105, 128, 150, 173, 196, 219 and 242. These values are kept fixed during the entire experiment, although the order of appearance of these 11 segments within the standard are scrambled pseudo-randomly. So the appearance of the standard varies from trial to trial. 

 	     
The screen design for two-alternate forced-choice experiment is shown in Fig. 6 (in the paper) for White illusion and SBC respectively.
In each trial, the subject has been first instructed to fix attention on a central red cross (1 deg within a 3.5 deg fixation window). 
Within one second the comparator and standard appears on the screen simultaneously, one of them centered at 7 deg to the left of the red cross and the other centered at 7 deg to the right of the red cross. Two vertical red lines are introduced on the comparator and standard at the same height of the red cross, which denotes the specific area of interest of them to be compared. 
The comparator and standard exists on the computer screen for about 3 seconds before disappearing. Subjects need not had to wait to give their judgments till the stimuli disappeared from the display. Red lines indicate the region of interest in the comparator to be judged against the nearest segment of the standard. If the comparator appears to be lighter than the standard, subjects have to press key number ONE, otherwise they have to press key number TWO. During one set of experiment (say for Simultaneous Brightness Contrast illusion), both the comparator (varying its width and length) and standard (by scrambling 11 intensity levels) are changed from trial to trial.

The perceived difference of brightness between the comparator and standard depends on the actual difference of brightness and also on the psychophysical response of the subject. To keep the subjects unbiased and attentive, various parameters were changed randomly from trial to trial. As an example, we can state that the comparator can appear to the left or right of the red cross, the intensity of the standard appearing at the same height of the comparator can vary widely etc.
Perceived difference of brightness between the comparator and the standard depends on the actual difference of brightness between those and also the psychophysical effect on the subject. If the actual difference in the brightness of the co-occurring comparator and the standard is zero, the apparent perceived difference is then entirely due to the psychophysical effect.

\subsection{Experimental Results}

The purpose of psychophysical experiment is to measure \textit{Point of Subjective Equality} (PSE)~\cite{mitra2018adaptive}, which is a measure involving actual intensities of the comparator and standard, when these appear to be same to the subject. 
In our experiments, the illusory enhancement or illusory decrement are measured at the point of subjective equality from the different sets of psychometric curves drawn for four different illusions. 
As always we measure the illusory effect of the darker target, we can calculate the average illusory decrement for each type of illusion under consideration.

Two sets of psychometric curves are presented in the paper. They represent the psychometric curves for Simultaneous Brightness Contrast (SBC) illusion and White illusion. 
We have performed similar experiments for other variants of illusions present in the dataset.
The psychometric curves for SBC, White illusion, gratings illusion and lower grid illusion are provided in Fig.~\ref{fig:psychometric_curve_supp}. Illusory decrement indicates the quantitative measure of perceived darkness. For example, given the standard grayscale value to be 150, illusory reduction of 32.95 indicates that the target is perceived to be grayscale value of 117.05 and looks darker. The illusory reduction of the same intensity comparator of grayscale value 150 for White illusion is maximum (49.22), for gratings illusion is minimum (27.11), and it lies within this maximum and minimum limit for SBC (35.03) and Lower-grid illusion (32.95) as shown in Fig.~\ref{fig:psychometric_curve_supp}. These psycophysical experiments statistically validate the dataset. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[scale=0.3]{figures/unet.png}
%\vspace{-0.2cm}
\caption{UNet architecture~\cite{ronneberger2015u}}
%\vspace{-0.2cm}
\label{fig:unet}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[scale=0.35]{figures/ill_1.png}
%\includegraphics[scale=0.35]{figures/ill_ex_sup.png}
%\vspace{-0.2cm}
\caption{Illusion examples: SBC (first column), White illusion (second column), Hermann grid (third column), grid illusion (fourth column) and grating illusion (fifth column) with varying grayscale values, scales and frequencies. These images are taken from our generated dataset to show the variety of scales, contrast and orientation.}
%\vspace{-0.2cm}
\label{fig:ill_example}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[scale=0.3]{figures/non_ill_ex_sup.png}
%\vspace{-0.2cm}
\caption{Non-illusion examples generated by us in the dataset by introducing non-linearity, dot-insertion~\cite{bakshi2020tiny,geier2008straightness} etc.}
%\vspace{-0.2cm}
\label{fig:non_ill_example}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Dataset}

\subsection{Dataset generation}
The dataset is generated by creating standard brightness illusions (i.e., SBC, White illusion, Hermann grid, upper and lower grid, grating illusion) with varying patch size, frequency, grayscale values as shown in Fig.~\ref{fig:ill_example}.
1149 non-illusion variants are also generated by utilizing several well-known results~\cite{bakshi2020tiny,geier2008straightness} as shown in Fig.~\ref{fig:non_ill_example}.
The dataset will be made public.


\section{Network details}
\subsection{Illuison identificaion}

For illusion identification, we finetune a ResNet-18 model. ResNet-18 is a convolutional neural network that is 18-layer deep~\cite{he2016deep}. The training has been done with stochastic gradient descent with learning rate of 0.01 and momentum of 0.9. 
We have also tried other variants like AlexNet~\cite{krizhevsky2012imagenet}(convolutional neural network containing 8 layers) and SqueezeNet~\cite{iandola2016squeezenet}(10 layer convolutional neural network with fewer parameters) to perform illusion identification and classification. The result is shown in Table 1 (in the paper).

\subsection{Illusion localization}

For illusion localization, we finetune a UNet architecture to segment out the perceived darkness. 
The UNet was designed by Ronneberger et al.~\cite{ronneberger2015u} for bio-medical image segmentation. The architecture contains two paths. The first path is the contraction path (also called as the encoder, refer to Fig.~\ref{fig:unet}) which is used to capture the context in the image.
The second path is the symmetric expanding path (also called as the decoder, refer to Fig.~\ref{fig:unet}) which is used to enable precise localization using transposed convolutions.
The exact architecture is shown in Fig.~\ref{fig:unet}.
The experimental details are given in Table 3 (in the main paper).
We consider a weighted combination of MSE loss ($L_{MSE}$ and SSIM loss ($L_{SSIM}$) as the loss function, $L = \alpha L_{MSE} + \beta L_{SSIM}$, where $L_{MSE}$ is mean squared error loss and $L_{SSIM}$~\cite{zhao2016loss} is the SSIM loss. We experimentally set the parameters, $\alpha = 0.4$, $\beta = 0.6$, which produced the best performance as shown in Tab.3 (in the main paper).
Adam optimizer is used for training with batch size of 32 and a learning rate of 0.001.
Some of the qualitative results on test images are shown in Fig.~\ref{fig:illustration}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
\centering
\includegraphics[scale=0.5]{figures/illustration.png}
%\vspace{-0.2cm}
\caption{Network response for illusion localization on test set: (a) test images, (b) corresponding groundtruth, (c) network response, (d) Binary response of the network by thresholding at 0.22. The trained network can localize perceived darkness quite efficiently.}
%\vspace{-0.2cm}
\label{fig:illustration}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[scale=0.3]{figures/step_sbc.png}
%\vspace{-0.2cm}
\caption{Network response for SBC with luminance gradient: illusion image (left), network response (right). Instead of binary background in SBC, the background has luminance gradient. The model still identifies the darker patch.}
%\vspace{-0.2cm}
\label{fig:step_SBC}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[scale=0.38]{figures/test3.png}
%\vspace{-0.2cm}
\caption{Network response for criss-cross brightness illusion: illusion image (left), network response (right). The darker patches are identified by the model.}
%\vspace{-0.2cm}
\label{fig:criss_cross}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[scale=0.66]{figures/todorovic.png}
%\vspace{-0.2cm}
\caption{Network response for todorovic illusion: todorovic illusion (left), network response (right). As the gray patch occludes by surrounding, the illusory effect is more focused in the center.}
%\vspace{-0.2cm}
\label{fig:todorovic}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[scale=0.33]{figures/cornsweet.png}
%\vspace{-0.2cm}
\caption{Network response for cornsweet illusion: cornsweet illusion (left), network response (right). The model correctly identifies the darker patch at the right.}
%\vspace{-0.2cm}
\label{fig:cornsweet}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[scale=0.3]{figures/bressan_1.png}
%\vspace{-0.2cm}
\caption{Network response for dungeon illusion: dungeon illusion (left), network response (right). The gray patches in the right looks darker, which the model correctly predicts. It also predicts Hermann grid blobs in the left side.}
%\vspace{-0.2cm}
\label{fig:bressan_1}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[!t]
% \centering
% \includegraphics[scale=0.3]{figures/bressan_2.png}
% %\vspace{-0.2cm}
% \caption{Network response for dungeon illusion variant 2: dungeon illusion variant 2 (left), network response (right).}
% %\vspace{-0.2cm}
% \label{fig:bressen_2}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[scale=0.45]{figures/benary_cross.png}
%\vspace{-0.2cm}
\caption{Network response for Benary's cross: Benary's cross (left), network response (right). The upper right gray patch seems to look darker, which the model correctly predicts.}
%\vspace{-0.2cm}
\label{fig:benary_cross}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Qualitative results on unseen illusions}

In this section, we verify the efficacy of our proposed data-driven approach on some more well-known illusions, which have not been used during training.
Qualitative network response for variants of dungeon illusion~\cite{bressan2001explaining} (Fig.~\ref{fig:bressan_1}), SBC with luminance gradient~\cite{poom2020influences} (Fig.~\ref{fig:step_SBC}), criss-cross brightness illusion~\cite{bressan2001explaining}(Fig.~\ref{fig:criss_cross}), Todorovic illusion~\cite{todorovic1997lightness}(Fig.~\ref{fig:todorovic}), benary's cross~\cite{gilchrist2014gestalt} (Fig.~\ref{fig:benary_cross}) and cornsweet illusion~\cite{poom2020influences} (Fig.~\ref{fig:cornsweet}) are shown here. These results suggest that the trained model can also correctly predict the perceived darkness on these type of unseen illusions.


\begin{table}[!t]
\centering
\scalebox{0.7}{
\begin{tabular}{|c|c|c|}
\hline
\textbf{Illusion} & \textbf{Accuracy} & \textbf{mIoU} \\ \hline
Hermann grid      & 0.6905            & 0.43          \\ \hline
Induced grating   & 0.9206            & 0.49          \\ \hline
Lower grid        & 0.7991            & 0.43          \\ \hline
Upper grid        & 0.8546            & 0.44          \\ \hline
SBC               & 0.8805            & 0.48          \\ \hline
White             & 0.9745            & 0.5           \\ \hline
\end{tabular}}
\caption{ \small Transferring illusions across other brightness illusions: testing on particular illusion as mentioned in the rows (from our dataset) while training the segmentation model for dark region localization on all other types except that particular illusion.}
\label{tab:ill_transfer}
\end{table}

\section{ Generalization to unseen illusions.}

To check whether the learned model generalizes among brightness illusions, we perform the following experiment. Among the five types of illusions, we train a segmentation network on four types of illusions and test on the unseen one. We show the results in Table.~\ref{tab:ill_transfer}. For example, we train on all the illusion images except the Hermann grid and test its generalization performance on the Hermann grid and observed illusion localization accuracy of 69.05\% with mIoU of 0.43 as shown in Table.~\ref{tab:ill_transfer}. We find that the learned segmentation model generalizes poorly when testing on the Hermann grid. However, for all other cases, the trained model transfers quite effectively for the other four types of illusions as shown in Table.~\ref{tab:ill_transfer}. We believe, as in the Herman grid, the illusory regions are not physically present and thus make the localization challenging.

Beyond these five types of illusion, we also evaluate of other popular unseen illusions such as Mach band illusion, non-linear Hermann grid, and Dungeon illusion. 

\textbf{Mach band illusion.}
Mach bands are apparent bright and dark lines occurring at the border between objects with different optical densities, contrast levels, or luminances~\cite{buckle2013now}.
Fig.~\ref{fig:mach_band} indicates that our learned model can detect Mach bands. Note, since we have trained to identify the darker patch, the learned model can identify the bright Mach band by displaying two surrounding parallel darker regions as shown in Fig.~\ref{fig:mach_band}.
% Mach band has several applications in medical imaging to identify lesions, fracture in radiology images as we will be discussing in Sec.~\ref{sec:application}.


\begin{figure}[!t]
   \begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[scale=0.25]{figures/mach_band.png}
    \vspace{-0.1cm}
    \caption{Mach band illusion (left) and corresponding learned model output (right). Two dark parallel dark patch indicates Mach band.}
    \vspace{-0.2cm}
    \label{fig:mach_band}
   \end{minipage}\hfill
   \begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[scale=0.23]{figures/dungeon_ill.png}
    \vspace{-0.3cm}
    \caption{Dungeon illusion and corresponding response form the network: Right region seems to be darker than left ones, however they are exactly the same grayscale level.}
    \vspace{-0.2cm}
    \label{fig:dungeon}
   \end{minipage}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Illusion vs natural image.}

We test illusion vs natural image (from the Caltech101 dataset~\cite{fei2004learning}) classification and achieve a high test accuracy of 99.98 \% in only 5 epochs.
% Thus, to make the problem non-trivial, we generate the non-illusion images by perturbing the illusions by following the common psychophysics techniques~\cite{bakshi2020tiny, geier2008straightness}. Note that the resulting non-illusion images are more visually similar to the illusion images than natural images.


\section{Test on illusions in natural images.} 

We test on natural images with diverse lighting and shading information which are used in illusion studies, e.g., Cartier-Bresson stimulus, as shown in Fig.~\ref{fig:nat_img_ill}~\cite{blakeslee2012spatial}. Our model can identify the darker regions and Mach bands in natural images as shown in Fig.~\ref{fig:nat_img_ill}.
We have also tested our framework with some of the recent approach of generating illusions from natural images~\cite{hirsch2020color}. Fig.~\ref{fig:nat_img_ill}(d) shows that our approach can identify illusory regions in those generated illusions too.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\vspace{-0.2cm}
\includegraphics[scale=0.22]{figures/nat_img_ill.png}
\vspace{-0.2cm}
\caption{Model response (lower row) on natural images (upper row): (a), (b), (c) natural images showing Mach band, (d) Illusory regions identified in illusions generated from natural image by ~\cite{hirsch2020color}.}
\vspace{-0.2cm}
\label{fig:nat_img_ill}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Network Analysis}

We investigate the feature maps learned by CNN models while identifying the illusions. We compute layer-wise attribution using GradCam~\cite{selvaraju2017grad} to analyze what features are encoded across the CNN layers. This approach, for a given target output, computes the contribution of the image regions for the final prediction across the layers. We use the Captum library~\cite{kokhlikyan2020captum} for computing the layer-wise attributions. We compare the layer-wise attributions of the ResNet model trained on natural images and trained on illusion images. 

In addition to the Gradcam attributes provided in the main paper, we are also providing some more examples of layer wise gradcam attributes for Hermann grid, SBC, non-illusion variant of Hermann grid and lower grid illusion in Fig.~\ref{fig:herman_grid_cam}, Fig.~\ref{fig:sbc_gradcam}, Fig.~\ref{fig:non_ill_gradcam} and Fig.~\ref{fig:lower_grid_gradcam} respectively.
As indicated in the main paper, there is a significant difference between the contribution of the image regions across the layers between the network trained with natural images (top row) and illusions (bottom row). 

In these examples also the lower layers tend to focus on low-level illusory features such as boundary between two regions with various intensities and the top layers learn more abstract features. The difference between the models trained with natural images and illusions are more prominent in the lower layers.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
%\vspace{-0.2cm}
\includegraphics[scale=0.265]{figures/grid_gradcam.png}
%\vspace{-0.2cm}
\caption[\small]{Gradcam attributes of the ResNet18 layers for the Hermann grid illusion. Upper row: model trained with natural images using the ImageNet dataset. Lower row: model trained with illusions. The layer attributes are clearly different for both these cases. Also, illusion finetuned model seems to capture the darker regions or patches in the lower layer response.}
%\vspace{-0.2cm}
\label{fig:herman_grid_cam}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
%\vspace{-0.2cm}
\includegraphics[scale=0.25]{figures/SBC_gradcam.png}
%\vspace{-0.2cm}
\caption[\small]{Gradcam attributes of the ResNet18 layers for SBC. Upper row: model trained with natural images using the ImageNet dataset. Lower row: model trained with illusions. The layer attributes are clearly different for both these cases. Also, illusion finetuned model seems to capture the darker regions or patches in the lower layer response.}
%\vspace{-0.2cm}
\label{fig:sbc_gradcam}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
%\vspace{-0.2cm}
\includegraphics[scale=0.25]{figures/non_ill_gradcam.png}
%\vspace{-0.2cm}
\caption[\small]{Gradcam attributes of the ResNet18 layers for the non-illusion variant of Hermann grid. Upper row: model trained with natural images using the ImageNet dataset. Lower row: model trained with illusions.}
%\vspace{-0.2cm}
\label{fig:non_ill_gradcam}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
%\vspace{-0.2cm}
\includegraphics[scale=0.25]{figures/lower_grid_gradcam.png}
%\vspace{-0.2cm}
\caption[\small]{Gradcam attributes of the ResNet18 layers for lower grid illusion. Upper row: model trained with natural images using the ImageNet dataset. Lower row: model trained with illusions.}
%\vspace{-0.2cm}
\label{fig:lower_grid_gradcam}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


